Constrained Bayesian Optimization with Max-Value Entropy Search

Bayesian optimization (BO) is a model-based approach to sequentially optimize expensive black-box functions, such as the validation error of a deep neural network with respect to its hyperparameters. In many real-world scenarios, the optimization is further subject to a priori unknown constraints. For example, training a deep network configuration may fail with an out-of-memory error when the model is too large. In this work, we focus on a general formulation of Gaussian process-based BO with continuous or binary constraints. We propose constrained Max-value Entropy Search (cMES), a novel information theoretic-based acquisition function implementing this formulation. We also revisit the validity of the factorized approximation adopted for rapid computation of the MES acquisition function, showing empirically that this leads to inaccurate results. On an extensive set of real-world constrained hyperparameter optimization problems we show that cMES compares favourably to prior work, while being simpler to implement and faster than other constrained extensions of Entropy Search.

==> benchmarking.tex <==
\section{Evaluation design}
\label{sec:evaluation-design}

We break down evaluation of competing methods and proposed optimization algorithm into two orthogonal parts.
Firstly, we discuss metrics by which all of the optimizers are compared. 
Secondly, we introduce a set of example blackboxes, that directly arise from practical applications of ML algorithms.

\subsection{Evaluation metrics}
For evaluation, we utilize ranking of optimizers across a set of example problems. 

We assume that no fixed budget is given, hence we average performances over a reasonably sized budget. For that, we triple the budget over which HPO overfits, and take that as a budget, see [reference!]. We use ranking, in order to compare the algorithms across functions with different output ranges. This gives rise to the following evaluation procedure.

All pairs of example blackboxes and optimizers are constructed; For every such pair, an optimizer is applied on a blackbox, and a best objective value is recorded for every iteration. Such procedure is repeated multiple times. Then, a rank of every algorithm is determined for every iteration on every blackbox, using Mann - Whitney statistical test to compare minima of different optimizers on same blackbox. Such rank is averaged across all blackboxes, and confidence bounds are derived. We derive both ranks over all iterations, as well average for specific iterations, and produce a plot.

\subsection{Example optimization problems considered}
We focus on domain of machine learning for our experiments, specifically on a task of hyperparameter optimization (HPO) of machine learning models. 

For our tuning tasks, we consider 7 [sage maker 1p] sklearn models, which are applied in both regression and classification domains.

For all of our supervised learning problems, we consider datasets from LibSVM repository [ref], from which we select 10 binary classification and 10 regression datasets. Names of the datasets are given in the description.

We consider the following HPO scenarios.
* Constrained memory optimization. In such scenario, we optimize AUC / coefficient of determination, subject to a constraint imposed on the size of the model. This models applications in IOT domain, where the size of the model is restricted. Alternatively, this models applications of large neural networks, that sometimes might not fit into the RAM of computing node. For simplicity and to make our results reproducible, we consider memory footprint of the model to be proportional to latency of inference.
* Sensitivity of a classifier, subject to specificity. This models applications such as in medical field, where it is more important to be accurate on one of the classes being classified. We consider a minority class in a dataset to be the most important one.
* Performance of regressor, subject to the largest error value. We consider a task where it is important to avoid catastrophic failures on any of the inputs, which is similar in spirit to above task.

Each of the constraints that we consider is imposed on some metric of a fitted model. We experiment with different thresholds on such metrics. We evaluate a number of random hyperparameter configurations on a task, to determine range of values of such metric. Let values of the metric be denoted as $m$. Note that we expect that for some thresholds, the global minimum is not affected; Let smallest such threshold be $m_{opt}$. For every blackbox function, we consider 3 thresholds: $\{ 0.5(m_{min}+m_{opt}) , m_{opt} , 0.5(m_{opt}, m_{max}) \}$. This tests scenarios where global optimium is inside the search space, and on the boundary.

Construction of such set results in (7*2*10*3) * 4 = 1680 possible constrained blackbox functions. We use a random subset of 50 blackboxes for our evaluations.

==> mes_comparison.tex <==
\begin{tabular}{lll}
\toprule
            Method & Avg. infeasible &  Avg. ranking \\
\midrule
       Standard BO &            70.3 &          12.4 \\
            Random &            39.3 &           7.1 \\
  MES $\delta=0.0$ &              21 &            12 \\
  MES $\delta=2.0$ &            19.6 &          10.8 \\
  MES $\delta=5.0$ &            16.1 &           7.8 \\
 MES $\delta=10.0$ &            25.3 &           6.4 \\
  CEI $\delta=0.5$ &            26.9 &           6.2 \\
  CEI $\delta=1.0$ &            20.8 &           5.3 \\
  CEI $\delta=4.0$ &            11.8 &           6.1 \\
 CEI $\delta=16.0$ &    \textbf{9.2} &             9 \\
         AP $p=50$ &            43.6 &           5.5 \\
         AP $p=75$ &            31.7 &  \textbf{4.3} \\
        AP $p=100$ &              17 &           4.5 \\
        AP $p=200$ &            14.9 &           5.8 \\
        AP $p=800$ &            16.6 &           8.5 \\
       AP $p=3200$ &            17.9 &           8.3 \\
\bottomrule
\end{tabular}


==> mes_hvh_comparison.tex <==
\begin{tabular}{lll}
\toprule
            Method & Avg. infeasible &  Avg. ranking \\
\midrule
       Standard BO &            70.3 &          12.8 \\
            Random &            39.3 &           7.7 \\
 CMES $\delta=-5.0$ &            41.9 &          11.8 \\
  CMES $\delta=0.0$ &            37.8 &           8.6 \\
  CMES $\delta=2.0$ &            27.4 &           7.1 \\
 CMES $\delta=10.0$ &            28.8 &  \textbf{4.0} \\
  CEI $\delta=0.5$ &            26.9 &           7.2 \\
  CEI $\delta=1.0$ &            20.8 &           5.8 \\
  CEI $\delta=4.0$ &            11.8 &           6.4 \\
 CEI $\delta=16.0$ &    \textbf{9.2} &           8.7 \\
         AP $p=50$ &            43.6 &           5.9 \\
         AP $p=75$ &            31.7 &           4.7 \\
        AP $p=100$ &              17 &             5 \\
\bottomrule
\end{tabular}


==> results.tex <==
\begin{tabular}{lcc}
             Optimizers & \% unfeasible & Avg rank \\
\hline
           $cMES, p=0.1$ &                           39.25 &             5.6 \\
           $cMES, p=0.5$ &                           41.41 &            5.57 \\
           $cMES, p=0.9$ &                           46.75 &   \textbf{5.17} \\
                  $cEI$ &                  24.26 &            6.14 \\
         $AP, perc.=50$ &                           49.63 &            6.13 \\
         $AP, perc.=75$ &                           36.62 &             6.1 \\
        $AP, perc.=100$ &                           27.87 &            5.77 \\
        $cEI_{observe}$ &                           35.54 &             6.1 \\
 $cMES_{observe}, p=0.1$ &                           46.73 &             6.7 \\
 $cMES_{observe}, p=0.5$ &                           48.93 &            6.51 \\
 $cMES_{observe}, p=0.9$ &                           53.23 &            6.21 \\
\hline
\end{tabular}


==> results_mes.tex <==
\begin{tabular}{lll}
\toprule
            Method & Avg. infeasible &  Avg. ranking \\
\midrule
       Standard BO &            70.3 &          12.4 \\
            Random &            39.3 &           7.1 \\
  MES $\delta=0.0$ &              21 &            12 \\
  MES $\delta=2.0$ &            19.6 &          10.8 \\
  MES $\delta=5.0$ &            16.1 &           7.8 \\
 MES $\delta=10.0$ &            25.3 &           6.4 \\
  CEI $\delta=0.5$ &            26.9 &           6.2 \\
  CEI $\delta=1.0$ &            20.8 &           5.3 \\
  CEI $\delta=4.0$ &            11.8 &           6.1 \\
 CEI $\delta=16.0$ &    \textbf{9.2} &             9 \\
         AP $p=50$ &            43.6 &           5.5 \\
         AP $p=75$ &            31.7 &  \textbf{4.3} \\
        AP $p=100$ &              17 &           4.5 \\
        AP $p=200$ &            14.9 &           5.8 \\
        AP $p=800$ &            16.6 &           8.5 \\
       AP $p=3200$ &            17.9 &           8.3 \\
\bottomrule
\end{tabular}


==> seq_comparison_table.tex <==
\begin{table}[]
\begin{tabular}{lllll}
                            & Random & GP Ignore & GP CEI & GP HVH Q=100\% \\
Failed evaluations rate, \% & 0.38   & 0.64      & 0.17   & 0.20           \\
Average ranking             & 1.25   & 3.0       & 1.75   & 0.5           
\end{tabular}
\caption{Comparison of various optimization methods in sequential setting. For every metric, less is better.}
\end{table}
